Far-Field Radiative Thermal Rectification with Bulk Materials

In this paper, we explore the far-field radiative thermal rectification potential of common materials such as metals, dielectrics and doped semi-conductors using radiative and thermo-radiative properties extracted from literature. Ten different materials are considered. The rectification coefficient is then calculated for 44 pairs of materials; each pair can be used for the two terminals of a radiative thermal diode. A thermal bias of 200 K is considered. The choice of materials and thermal bias value is only bound by data availability in literature. Obtained results, highlight new candidate materials for far-field radiative thermal rectification. They also highlight materials where thermal rectification is not negligible and should be considered with care in heat transfer calculations when considering systems subject to a comparable thermal bias and where these materials are used. Among the materials studied, undoped Indium Arsenide (InAs) shows great promise to be employed for thermal rectification, with a thermal rectification ratio reaching 90.5% in combination with other materials. Obtained results pave the way for an optimized design of thermal radiation control and management devices such as thermal diodes.

==> 00README.XXX.tex <==
nohypertex
